Spatial Name System

The development of emerging classes of hardware such as Internet of Thing devices and Augmented Reality headsets has outpaced the development of Internet infrastructure. We identify problems with latency, security and privacy in the global hierarchical distributed Domain Name System. To remedy this, we propose the Spatial Name System, an alternative network architecture that relies on the innate physicality of this paradigm. Utilizing a device's pre-existing unique identifier, its location, allows us to identify devices locally based on their physical presence. A naming system tailored to the physical world for ubiquitous computing can enable reliable, low latency, secure and private communication.

==> sections/0.1_title_page_anonymised.tex <==

{\sffamily
\begin{titlepage}
	\makeatletter
	% University logo with shield
	\hspace*{-14mm}\includegraphics[width=65mm]{logo-dcst-colour}
	
	\begin{Large}
		\vspace{20mm}
		Research project report title page
		
		\vspace{35mm}
		Candidate 2102J
		
		\vspace{42mm}
		\textsl{``\@title''}
	\end{Large}
\end{titlepage}
}

==> sections/7_appendices.tex <==
\begin{appendices}

\chapter{Appendix}
\label{ch-appendix}

\end{appendices}

